SciLit: A Platform for Joint Scientific Literature Discovery, Summarization and Citation Generation

Scientific writing involves retrieving, summarizing, and citing relevant papers, which can be time-consuming processes in large and rapidly evolving fields. By making these processes inter-operable, natural language processing (NLP) provides opportunities for creating end-to-end assistive writing tools. We propose SciLit, a pipeline that automatically recommends relevant papers, extracts highlights, and suggests a reference sentence as a citation of a paper, taking into consideration the user-provided context and keywords. SciLit efficiently recommends papers from large databases of hundreds of millions of papers using a two-stage pre-fetching and re-ranking literature search system that flexibly deals with addition and removal of a paper database. We provide a convenient user interface that displays the recommended papers as extractive summaries and that offers abstractively-generated citing sentences which are aligned with the provided context and which mention the chosen keyword(s). Our assistive tool for literature discovery and scientific writing is available at https://scilit.vercel.app

==> bkup.tex <==
% it remains a challenge to make these large corpora searchable efficiently for the benefit of researchers in in finding literature and writing articles. 
% We propose \textsc{SciLit}, a platform for efficient retrieval of papers from multiple large-scale scientific corpora with a two-stage prefetching-reranking architecture.
% In the prefetching phase, documents are first filtered based on a given lexical syntax and then sorted by an embedding-based nearest neighbor search engine. In the reranking phase, the prefetched documents are further scored and ranked by a fine-tuned BERT model.
% With a hierarchical architecture for document search,
% \textsc{SciLit} allows easy plugging and unplugging of paper databases and  real-time PDF indexing, demonstrating a high  degree of scalability and flexibility.

    % uploading PDFs to create a personal bibliography to search for papers, 

% This is especially helpful when we providing background information or comparing the results with related works.
% This process is common scenario in scientific writing 
% In today's era of information overload where the literature is growing rapidly \cite{hoq2014information}, 

% or to dynamically index uploaded PDFs in real time, which potentially allows users to search the literature and apply summarization algorithms to it within their personal libraries.


%finding, reading, summarizing relevant papers, extracting the main points, and writing sentences that cite and summarize the paper is a common but time-consuming process, in part because there is a large amount of literature that requires one's attention to select, read, understand, and summarize the lengthy content. 
%To facilitate this process and reduce authors' workload when writing, 

%\textsc{SciLit} efficiently recommends papers from large databases of hundreds of millions of papers, backboned by a two-stage prefetching-reranking literature retrieval system, 
%aggregated from recently released scientific corpora such as S2ORC, 
%and it allows easy plugging and unplugging of paper databases and real-time PDF indexing, demonstrating a high degree of scalability and flexibility.




% Scientific literature is an important resource to consult when we are following up on an idea, searching for background information on a fact, or searching for supporting and conflicting information on a claim, or most often when we want to learn something new about a topic \cite{lindsay1999literature}. 
 
% For researchers,
% This large corpora are valuable resources for text mining, e.g. obtain papers from a certain field of study, obtaining the citation information dataset. For authors, these are  valuable knowledge base for researchers looking for documents while writing articles. However, in practice, it is not easy to efficiently to start use this multiple large corpora



This corpora has large size - an efficient indexing and document retrieval system

This corpora has various format - a uniform yet flexible data structure storing information of each paper

In the meantime, much progress has been made in the domain natutal language domain. Especially in the field of information retrieval and document summarization. For example,


In order to make better use of these corpora for text mining research, or as a valuable knowledge base for researchers looking for documents while writing articles, an integrated literature discovery platform is necessary, which we deem needs to meet the following requirements to be used in practical scenarios.

Capable of parsing, storing, indexing and displaying papers from multiple corpora with various data formats. For example, the content of each paper in S2ORC is stored in json format with dedicated fields. papers in BioRxiv \cite{sever2019biorxiv} are stored in XML format. And the papers in the general index do not have full text, but a package of n-grams.

% Third, When providing service to users, Users may have the need to upload and index their PDFs so that they can perform literature search within their personal bibliographies.

To cope with these requirements, we propose \textsc{SciLit}, a microservcie-based platform designed for searching for papers from multiple large corpora and easy extension of other nlp-driven functions.

To efficiently retrieve papers from 


To cope with these requirements, we propose \textsc{SciLit}, a microservcie-based platform designed for searching for papers from multiple large corpora and easy extension of other nlp-driven functions.

To efficiently retrieve papers from 


To cope with these requirements, we propose \textsc{SciLit}, a microservcie-based platform designed for searching for papers from multiple large corpora and easy extension of other nlp-driven functions.

To efficiently retrieve papers from 


% requires authors effort on selecting relevant papers from enormous volume of scientific literature and compose texts analytically summarizing the paper
% read, understand, and summarize the lengthy007
% content. 

much work for ones to go through literature, select matched candidate, read the content of the paper, and finally write a   which raise a question whether it is possible to faciliate the process.

% common scenario: when we write a sentence, such as


.  In the prefetching phase, documents are first ranked using efficient retrieval algorithms including sparse retrieval methods such as BM25 that relies on a huge and spare inverted index or dense retrieval methods that map documents and queties into dense vector representation and ranks document according to the cosine or Euclidean distance between query and document embeddings. In the reranking phase, the prefetched documents are further scored and ranked by a fine-tuned BERT model. 


% These corpora are not only valuable resources for text mining research \cite{hotho2005brief},
% % such as accessing papers in a particular research area or extracting citation information from a corpus, 
% but they are also a promising valuable knowledge base for authors looking for literature when writing articles.

% However, in practice, it is not easy to start using these large corpora 

Yet its scalability is still understudied when the database size scales to hundreds of millions.



In the prefetching phase, documents are first filtered based on a given lexical syntax and then sorted by an embedding-based nearest neighbor search engine. 
In the reranking phase, the prefetched documents are further scored and ranked by a fine-tuned BERT model.

Recent work in text retrieval on large database typically utilize two-sta  


Recently, 
Recent progress in text retrieval, embedding-based KNN, 

dense representation, more storage/memory efficient, easy to accelerate with parallization / GPU speedup. 
Efficient prefetching + deep reranking has been applied in text retrieval task such as citation recommendation, which achieved a good balance between accuracy and query speed, which make it possible to effiently index and search from millions of documents. 
Progress in document summarization. Dancer, MemSum, efficient summarization transformer, 
Citation generation, pilot study BACO. 




    Efficient document retrieval from massive corpora of hundreds of millions of papers, such as S2ORC containing over 136 million papers \cite{lo-wang-2020-s2orc}, and General Index containing over 100 million papers 


   Easy to dynamically update the indexing system to respond to potential changes in the database, including adding or removing certain corpora and incremental updates such as daily digestion of available new papers and real-time indexing of user-uploaded PDFs.

Extensible architecture to incorporate additional NLP-driven features such as keyword suggestions, extractive document summarization, and reference text generation that have the potential to help users in the literature understanding and scientific writing process, and support easy plug-and-play to add, remove, or update algorithms.


% To this end, we propose \textsc{SciLit}, a microservice-based platform designed to search papers from multiple large corpora and easily extend other natural language processing (NLP)-driven features.
% which is 1) Efficient document retrieval from massive; 2)  Easy to dynamically update the indexing system to respond to potential changes in the database, including adding or removing certain corpora and incremental updates such as daily digestion of available new papers and real-time indexing of user-uploaded PDFs. 3) pport easy plug-and-play to add, remove, or update algorithms. 

show case


Recent advances in the release of scientific open research corpora \cite{lo-wang-2020-s2orc, else2021giant}, as well as research on information retrieval \cite{guo2020deep} and document summarization \cite{yao2017recent,koh2022empirical} algorithms, shed light on possible answers to this question.


 from the vast open research corpora, such as S2ORC \cite{lo-wang-2020-s2orc} with over 136 million papers and General Index \cite{else2021giant}  with over 100 million records.


% For example, a two-stage prefetching-reranking strategy \cite{bhagavatula2018content} is commonly used to strike a good balance between speed and accuracy when recommending papers from a database of millions of papers.
% Documents are first prefiltered using an efficient retrieval algorithm such as BM25 \cite{robertson2009probabilistic,keller2021tekma} or dense embedding-based nearest neighbor search \cite{10.1145/3486250, gu2022local}, and then scored and reranked by a fine-tuned large-scale language model such as BERT \cite{devlin-etal-2019-bert}.

%  \cite{lo-wang-2020-s2orc, else2021giant},  \cite{guo2020deep} \cite{yao2017recent,koh2022empirical} algorithms,


% For example, \citet{gu-etal-2022-memsum} proposed an extractive summarization model to extract the abstract of a scientific paper by repeatedly selecting sentences in a Markov decision process and using the extracted sentences as highlighted sentences to help readers capture the main content of the paper. 
% \citet{xing_automatic_2020} first proposed to generate citation sentences using the contextual text surrounding the citation sentence and the abstract of the paper intended to be cited, and this model was further enhanced by citation network information in~\citet{ge_baco_2021,wang_disencite_2022}.


, and external knowledge such as citation network information
% that can serves as the highlights to help readers grasp the main points, and recent work \citet{xing_automatic_2020} has explored the possibility of generating citation sentences based on the contextual text surrounding the citation sentence, the abstract of the target paper, and external knowledge such as citation network information \cite{ ge_baco_2021,wang_disencite_2022}.

that includes an efficient literature retrieval module, an extractive summarization module, and a citation text generation module to help users search for relevant papers or find recommendations, automatically extract highlights and generate reference text in a one-stop manner, and it can be easily extended with other natural language processing (NLP)-driven features.


% In order to organize and structure documents from different scientific corpora,  
% % organizing and structuring scientific documents, which will be useful for developers who want to build their own database of scientific papers,

When importing scientific corpora into our databases, we dump each corpus into a separate SQLite\footnote{\url{https://www.sqlite.org}} database to flexibly place and deploy the prefetching server at different physically locations. In addition,
we process documents from different corpora into a uniform JSON structure with dedicated fields, including “Title”, “Author” and “PublicationDate”, etc. for the metadata, and “Content.Abstract\_Parsed”,  “Content.Fullbody\_Parsed” for the parsed full text, which allows to index, query, summarize and display documents from different corpora with the same code base.
The detail of the JSON schema is shown in Appendix XXX. 



% The statistics of the databases we currently aggregated are listed in Table \ref{}.
% Paper ID system

add
These index files will enable developers to build an efficient information retrieval system that can use the inverted index to perform keyword boolean filtering on related documents and use the embedding index to further rank filtered documents based on textual semantic similarity.


% one is for hierarchical ranking and on is scibert (compare these two on retrieval tasks) We fine-tune a SciBERT model to take the local/global context and paper's title abstract as input following \cite{gu_local_2022}.
% We fine-tune a SciBERT model to take the local/global context and paper's title abstract as input following \cite{gu_local_2022}.
% We fine-tune a SciBERT model to take the local/global context and paper's title abstract as input following \cite{gu_local_2022}.

% We choose the summary to be extractive instead of abstractive to prevent readers from being mislead by potential hallucinations introduced in abstractive summarization models

% The front-end user interface communicates with the back-end through an api gateway.
% The api gateway receive all requests from the frontend, route them to corresponding downstreaming microservices, collect returned values and send them back to the frontend. 


such as literature discovery, extracting highlights or generating citation sentences. In particular, the literature discovery service dispatches queries first to a prefetching service that maintains multiple indexing files, and then send the query as well prefetched paper IDs to the reranking service. A database interface service manages databases for multiple scientific corpora and provide s unified interface for accessing papers' content given the identifier.


% Such a modularized architecture allows us to easily add or remove databases. For example, we can add a new database storing user-uploaded papers and  to the database interface and connect the corresponding indexing files to the prefetching service, to enable 
% update the data

% which makes it easy to upgrade the backend system without stopping. E.g. add/remove database, create a PDF indexing service, etc. 


% In the back-end, each module is wrapped into a microservice.
% Microservices communicate via Flask POST requtes.  
% Each microservice runs relative independently, which makes the update of each module add-hoc without influence other subsystems.
% Each server run independetly, easily add/remove new servcers. For example, PDF parsing, we can create an database holding user uploaded papers and indexing PDFs, so that users can create a personal library by uploading PDFs from their local computer, we will process the PDF with doc2json \cite{}, converting into our json schema, indexing them. We believe this is especially useful when users have a large collection of biblography to maintain, sometimes it is even difficult to find a paper in our biblography.
% We introduce a special field Uploader to control the visibility to make sure the uploaded PDFs are only searchable to the owner (uploader), making it a private libarary search manager.

% The uploading/indexing is running in real-time fast without disturbing our functionality, like serach or sumamrize

% We create the training dataset by mining XXX training pairs from the database.



% \begin{itemize}
%     \item What  Citation Generation  module does?
%     \item what is the difference between other work?
%     \item how this is achieved? Model structure? How to train?
    
% \end{itemize}

% \begin{itemize}
%     \item What  Citation Generation  module consists of?
% \end{itemize}


% \subsection{Databases}
%  1. json schema
%  2. Sqlite Databse, 
%  3. Paper ID system
 
%  A JSON schema illustrating the data structure of each scientific publication document stored in our database will be documented, including the following details: i. All the available fields for each document, such as “Title”, “Author” and “PublicationDate” for the metadata, and “Content.Fullbody\_Parsed” for the parsed full text; and ii. How the full text is parsed and stored in our database.
% We believe this JSON schema will provide a good template for how to organizing and structuring scientific documents, which will be useful for developers who want to build their own database of scientific papers, or for aggregating more publications for our database.

% A complete dump of all our aggregated open access scientific publications will be made available for developers to download for free. Our aggregated scientific publications will be stored using an SQLite database because of its advantages of easy deployment and native support for Python.

% Preprocessing codes include the following aspects:
% i) document parsing: parsing the raw document from different collections such as S2ORC, Crossref, arXiv, bioRxiv, PubMed, and converting the parsed document into the standardized data structure defined by the JSON schema;
% ii) SQLite database interface, to implement the database operation including getting papers, inserting papers, and updating papers.

 
% \subsection{Indexing}

% Along with the scientific publications SQLite database, we will provide the index files that enable developers to efficiently filter and rank specific documents. 
% These index files contain two parts. The first part is an inverted index that stores a mapping table. Given a word, it records the paper IDs of all publications that contain this word, where the paper IDs can be used to retrieve the content of the publication from the SQLite database we provide. The second part is an embedding index that contains the embedding, a 256-dimensional vector representation, of each scientific publication in our database, computed by an efficient text encoding model Sent2vec (Pagliardini et al 2017). 
% These index files will enable developers to build an efficient information retrieval system that can use the inverted index to perform keyword boolean filtering on related documents and use the embedding index to further rank filtered documents based on textual semantic similarity, similar to the discovery engine of our current Science Editor platform.


% Codes for document ranking will include our implementation of an efficient brute-force nearest neighbor search module which is able to rank more than 100 million paper embeddings efficiently. It is designed to have the following features:
% i) multiple-processing brute-force nearest neighbor search;
% ii) mixed-precision (bool, int4, int8, float32) GPU computation to speed up the ranking operation.
% Estimated Time: 6 months
% Moreover, we will write a publication describing the whole pipeline of data aggregation, processing, indexing, and setting up a discovery system. This publication will be of course freely accessible.
%                       Estimated Time: 12 months



\textsc{SciLit} consists of three main modules (): 1) the literature discovery module, 2) the extractive summarization module and 3) the citation generation module. We describe the implementation details of these modules in this section.


In this work we use up to six preceding sentences that are within the same section as the citation sentence as the context.

%first filtering the documents based on the provided keywords, and then ranking the filtered documents based on the cosine similarity of the query embedding and the document embedding to obtain the top K candidate documents. 

% We constructed triplet pairs (query, cited paper, uncited paper) from the scientific corpus to fine-tune SciBERT reranker to encourage affinity scores between queries and cited papers, while penalizing affinity scores for uncited papers.

% Although BERT-based extractive summarizers \cite{XXX} have achieved the state-of-the-art on popular document summarization benchmarks such as CNN/DM and NYT \cite{XXX}, these models usually have a strict length limit of input token, typically 512 \cite{} or 768 \cite{}, due to the computation intensity of the transformer structure \cite{XXX}. Such a limit makes it not feasible to summarize scientific papers that can easily exceeds the length limit above. 
% BERT-based extractive summarizers \cite{jia-etal-2020-neural,zhong-etal-2020-extractive} have achieved state-of-the-art results on popular document summarization benchmarks such as CNN/DM \cite{NIPS2015_afdec700} and NYT \cite{sandhaus2008new}. However, due to the high computational intensity of the transformer structure, these models usually have a hard limit on the length of the input tokens, typically 512 \cite{zhong_extractive_2020} or 768 \cite{jia-etal-2020-neural}.
% This limitation makes it infeasible to use these BERT-based extractive summarizers to summarize long scientific papers.

% Recently, BERT-based extractive summarizers \cite{https://doi.org/10.48550/arxiv.1903.10318,jia-etal-2020-neural,zhong-etal-2020-extractive} usually have a hard limit on the length of the input tokens, typically 512  or 768, which makes it infeasible to summarize long scientific papers.

% During an extraction process, an agent decides which sentence to select next or to stop extracting based on the state of the already extracted sentences.
% MemSum can summarize long document summarizing long document without exhaust GPU memory due to a light-weight model structure, and is computationally efficient, summarizing a paper within only 30 ms. These features make it suitable model for our extractive summarization module. Here We used the MemSum model trained on the PubMed dataset \cite{}.


% \begin{itemize}
%     \item What extractive summarization module does?
%     \item what is the main concern? document length, summarization speed?
%     \item how this is achieved? what model is used? how the model is trained?
% \end{itemize}

% \begin{itemize}
%     \item What extractive summarization module consists of?
% \end{itemize}

% Conceptually, if we consider the human brain as a citation text generator, then the keyword "MAX pooling" should be used as a thematic cue for the citation sentence generation, which also applies to the automatic citation generation model.

% The literature discovery service first sends the query to the prefetching service, which collects the prefetched paper IDs from all indexing systems and removes duplicates, then sends the query and the prefetched IDs to the reranking service, gets the reranked IDs and returns them to the API gateway.

% We compared MemSum with 
% two baselines: 1) Lead-10, selecting first 10 sentences from the full body as the highlights; 2) 
% BertSum \cite{https://doi.org/10.48550/arxiv.1903.10318}, a Bert-based summarizer that truncates long documents into 512 tokens before extraction.

%Another AI-driven platform focuses on extractive text summarization, which combines rhetorical sentence classification and extractive text summarization tasks #CIT.

%Recently, AI-driven platforms focused on literature recommendation and summarization have been proposed, respectively. One such platform is AI Research Navigator \#CIT, which combines classical keyword search with neural retrieval to discover and organize relevant literature.


%Recently, platforms focusing on literature search and analysis haven proposed. The AI Research Navigator \#CIT platform combines classical keyword search with neural retrieval to discover and organize relevant literature.

%[CIT] Fadaee, Marziehet al. “A New Neural Search and Insights Platform for Navigating and Organizing AI Research.” (2020).


%A content-based literature recommendation system for datasets is a part of the dataset reusability platform developed at the University Texas Health Science Center at Houston for datasets related to gene expression \#CIT.


% [CIT] Patra, Braja Gopal, et al. “A Content-Based Literature Recommendation System for Datasets to Improve Data Reusability – A Case Study on Gene Expression Omnibus (GEO) Datasets.” Journal of Biomedical Informatics, vol. 104, Apr. 2020, p. 103399. Crossref, https://doi.org/10.1016/j.jbi.2020.103399.


%For example, AI Research Navigator \#CIT combines classical keyword search with neural retrieval to discover and organize relevant literature. Zeta Alpha.


% [CIT] Fadaee, Marziehet al. “A New Neural Search and Insights Platform for Navigating and Organizing AI Research.” (2020).

%For example, Embedding-based Scientific Literature Discovery in a Text Editor application \#CIT combines Boolean keyword filtering with nearest neighbor search over text embeddings, providing a discovery experience tuned to an author's manuscript and his interests.


% [CIT] Gökçe, Onuret al. “Embedding-based Scientific Literature Discovery in a Text Editor Application.” (2020).


When
When generating each sentence, all text including generated sentences before it rae trated as context and keywords in shown in the bracket.


